AxOMaP: Designing FPGA-based Approximate Arithmetic Operators using Mathematical Programming

With the increasing application of machine learning (ML) algorithms in embedded systems, there is a rising necessity to design low-cost computer arithmetic for these resource-constrained systems. As a result, emerging models of computation, such as approximate and stochastic computing, that leverage the inherent error-resilience of such algorithms are being actively explored for implementing ML inference on resource-constrained systems. Approximate computing (AxC) aims to provide disproportionate gains in the power, performance, and area (PPA) of an application by allowing some level of reduction in its behavioral accuracy (BEHAV). Using approximate operators (AxOs) for computer arithmetic forms one of the more prevalent methods of implementing AxC. AxOs provide the additional scope for finer granularity of optimization, compared to only precision scaling of computer arithmetic. To this end, designing platform-specific and cost-efficient approximate operators forms an important research goal. Recently, multiple works have reported using AI/ML-based approaches for synthesizing novel FPGA-based AxOs. However, most of such works limit usage of AI/ML to designing ML-based surrogate functions used during iterative optimization processes. To this end, we propose a novel data analysis-driven mathematical programming-based approach to synthesizing approximate operators for FPGAs. Specifically, we formulate mixed integer quadratically constrained programs based on the results of correlation analysis of the characterization data and use the solutions to enable a more directed search approach for evolutionary optimization algorithms. Compared to traditional evolutionary algorithms-based optimization, we report up to 21% improvement in the hypervolume, for joint optimization of PPA and BEHAV, in the design of signed 8-bit multipliers.

==> 999_bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{imgs/sss_1.JPG}}]
    {Siva Satyendra Sahoo} is currently working as a R\&D Engineer with at IMEC, Leuven.  He received his doctoral degree (Ph.D., 2015-2019) in the field of reliability in heterogeneous embedded systems from the National University of Singapore, Singapore. He completed his masters (M.Tech, 2010-2012) from the Indian Institute of Science, Bangalore in the specialization Electronics Design Technology. He has also worked with Intel India, Bangalore in the domain of Physical Design. His research interests include Embedded Systems, Machine Learning, Approximate Computing, Reconfigurable Computing, Reliability-aware Computing Systems, and System-level Design. For the presented work, he was working as Postdoctoral Researcher with the Chair for Processor Design at TU Dresden.
\end{IEEEbiography}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{imgs/liu.JPG}}]{Qunyou Liu} is a Ph.D. student at the Embedded system Laboratory, Swiss Federal Institute of Technology Lausanne. He has completed his BSc in Electrical Engineering from the China University of Petroleum, China. From 2019 to 2022, he is master student at Technische Universit{\"a}t Dresden. His current research interests include the Computer architecture, machine learning and system level design. 
% \end{IEEEbiography}


% \begin{IEEEbiography}%[{\includegraphics[width=1in,height=1.25in,clip]{imgs/amm_imm.JPG}}]
%     {Amritha Immaneni} . 
% \end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{imgs/salim.JPG}}]
    {Salim Ullah} is a Postdoctoral Researcher at the Chair for Processor Design, Technische Universit{\"a}t Dresden. He has completed his BSc and MSc in Computer Systems Engineering from the University of Engineering and Technology Peshawar, Pakistan. His current research interests include the Design of Approximate Arithmetic Units, Approximate Caches, and Hardware Accelerators for Deep Neural Networks. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.95in,height=1.25in,clip]{imgs/akash.JPG}}]
    {Akash Kumar} (SM’13) received the joint Ph.D. degree in electrical engineering and embedded systems from the Eindhoven University of Technology, Eindhoven, The Netherlands, and the National University of Singapore (NUS), Singapore, in 2009. From 2009 to 2015, he was with NUS. He is currently a Professor with Technische Universität Dresden, Dresden, Germany, where he is directing the Chair for Processor Design. His current research interests include the design, analysis, and resource management of low-power and fault-tolerant embedded multiprocessor systems.
\end{IEEEbiography}
